Phantom Edges in the Problem Hamiltonian: A Method for Increasing Performance and Graph Visibility for QAOA

The Quantum Approximate Optimization Algorithm (QAOA) is a variational quantum algorithm that can be used to approximately solve combinatorial optimization problems. However, a major limitation of QAOA is that it is a "local" algorithm for finite circuit depths, meaning it can only optimize over local properties of the graph. In this paper, we present Phantom-QAOA, a new QAOA ansatz that introduces only one additional parameter to the standard ansatz -- regardless of system size -- allowing QAOA to "see" more of the graph at a given depth $p$. We achieve this by modifying the target graph to include additional $\alpha$-weighted edges, with $\alpha$ serving as a tunable parameter. This modified graph is then used to construct the phase operator and allows QAOA to explore a wider range of the graph's features. We derive a general formula for our new ansatz at $p=1$ and analytically show an improvement in the approximation ratio for cycle graphs. We also provide numerical experiments that demonstrate significant improvements in the approximation ratio for the Max-Cut problem over the standard QAOA ansatz for $p=1$ and $p=2$ on random regular graphs up to 16 nodes.

==> cycle_graphs.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{0.48\columnwidth}  % Adjusted to fit within the column width
        \centering
        \begin{tikzpicture}[scale=1]
            % Draw the 8-vertex cycle graph in red
            \foreach \i in {1,2,...,8} {
                \node[circle, draw, fill=white] (N\i) at (\i*45:1.5) {};
            }
            \foreach \i in {1,2,...,8} {
                \pgfmathtruncatemacro{\j}{mod(\i,8) + 1}
                \draw[red] (N\i) -- (N\j);
            }

            % Draw the Hamiltonian cycle in the complement graph in green
            \draw[green] (N1) -- (N4);
            \draw[green] (N4) -- (N7);
            \draw[green] (N7) -- (N2);
            \draw[green] (N2) -- (N5);
            \draw[green] (N5) -- (N8);
            \draw[green] (N8) -- (N3);
            \draw[green] (N3) -- (N6);
            \draw[green] (N6) -- (N1);
        \end{tikzpicture}
    \end{minipage}
    \hfill
    \begin{minipage}[t]{0.48\columnwidth}  % Adjusted to fit within the column width
        \centering
        \begin{tikzpicture}[scale=1]
            % Draw the 8-vertex cycle graph in red
            \foreach \i in {1,2,...,8} {
                \node[circle, draw, fill=white] (N\i) at (\i*45:1.5) {};
            }
            \foreach \i in {1,2,...,8} {
                \pgfmathtruncatemacro{\j}{mod(\i,8) + 1}
                \draw[red] (N\i) -- (N\j);
            }

            % Draw the Hamiltonian cycle in the complement graph in green, hopping two nodes over
            \draw[green] (N1) -- (N3);
            \draw[green] (N3) -- (N5);
            \draw[green] (N5) -- (N7);
            \draw[green] (N7) -- (N1);
            \draw[green] (N2) -- (N4);
            \draw[green] (N4) -- (N6);
            \draw[green] (N6) -- (N8);
            \draw[green] (N8) -- (N2);
        \end{tikzpicture}
    \end{minipage}
    \caption{\footnotesize Examples of 8-vertex cycle graphs $G$ shown in red and additional edges from the complement graph $\overline{G}$ shown in green. The left image shows a $G'$ that is still regular and triangle-free, while the right image shows a $G'$ that is still regular and now contains triangles.}
    \label{fig:combined_graphs}
\end{figure}
